Load Modulation for Backscatter Communication: Channel Capacity and Near-Capacity Schemes

In backscatter communication (BC), a passive tag transmits information by just affecting an external electromagnetic field through load modulation. Thereby, the feed current of the excited tag antenna is modulated by adapting the passive termination load. This paper studies the achievable information rates with a freely adaptable passive load. As a prerequisite, we unify monostatic, bistatic, and ambient BC with circuit-based system modeling. We present the crucial insight that channel capacity is described by existing results on peak-power-limited quadrature Gaussian channels, because the steady-state tag current phasor lies on a disk. Consequently, we derive the channel capacity for the case of an unmodulated external field, for general passive, purely reactive, or purely resistive tag loads. We find that modulating both resistance and reactance is important for very high rates. We discuss the capacity-achieving load statistics, rate asymptotics, technical conclusions, and rate losses from value-range-constrained loads (which are found to be small for moderate constraints). We then demonstrate that near-capacity rates can be attained by more practical schemes: (i) amplitude-and-phase-shift keying on the reflection coefficient and (ii) simple load circuits of a few switched resistors and capacitors. Finally, we draw conclusions for the ambient BC channel capacity in important special cases.

==> AP-AmbientMRC.tex <==
The ambient backscatter case requires special care because the voltages $v\Tx\Ind$ and $v\Rx\Ind$ may exhibit fast time-variations from modulation.
In that regard, we require the following conditions:
%(i) All relevant propagation channels (tag $\rightarrow$ receiver, ambient source $\rightarrow$ tag, ambient source $\rightarrow$ receiver) either do not suffer from fading at all or they are subject to slow fading.
\mbox{(i) The} relevant propagation channels are either subject to block fading or no fading at all.
(ii) There is only a single ambient source and it uses digital modulation.
(iii) The channel from ambient source to receiver is much stronger than the backscatter channel, i.e. $\EV{|Z\RxTx i\Tx|^2} \ll \EV{|v\Rx\Ind|^2}$.
(iv) The modulated signal $v\Rx\Ind$ can be decoded correctly.
(v) There is no interference from other backscatter tags.

We identify the following different cases for which the channel capacity result \Cref{eq:Capacity} applies to ABC in some fashion:

\textbf{1.) The ambient source has much faster symbol rate than the load modulation:} Let $L \gg 1$ denote the ratio of symbol rates and assume $L \in \bbN$. We consider the fast symbol rate with time index $\ell$. Let $s[\ell] := \f{-Z\RxTx}{R\Tx(1 + z[\ell])} v\Tx\Ind[\ell] + v\N[\ell]$, which is $v$ after compensation of the decoded $v\Rx\Ind[\ell]$. The modulated $v\Tx\Ind[\ell]$ is i.i.d. random and $v\N[\ell] \iid \mathcal{CN}(0,\sigma^2 L)$ while $z[\ell]$ is constant over length-$L$ blocks. For a specific block %we denote the constant $z[\ell]$ as $z$ and
we collect the various signals in the vectors ${\bf s}, {\bf v}\Tx\Ind, {\bf v}\N \in \bbC^L$ to write
${\bf s}
%= -Z\RxTx {\bf i}\Tx + {\bf v}\N
= \f{-Z\RxTx}{R\Tx(1 + z)} {\bf v}\Tx\Ind + {\bf v}\N$.
We consider maximum-ratio combining
$\tilde{y} = - {\bf u}\H {\bf s} / \sqrt{L}$ at the receiver, whereby
${\bf u} := {\bf v}\Tx\Ind / \|{\bf v}\Tx\Ind\|$.
This results in the relation $\tilde{y} = \f{Z\RxTx}{R\Tx(1 + z)} \|{\bf v}\Tx\Ind\| / \sqrt{L} + \omega$ with $\omega \sim \mathcal{CN}(0,\sigma^2)$. This relation is equivalent to the signal model \Cref{eq:SignalModel} with the exception that $|v\Tx\Ind|$ is replaced by $\|{\bf v}\Tx\Ind\| / \sqrt{L}$. The latter approaches the RMS value of $v\Tx\Ind$ for large $L$. Therefore the system behaves as if $v\Tx\Ind$ was constant.

\textbf{2.) The ambient source has much slower symbol rate than the load modulation:} The effect on the backscatter system is the same as if $v\Tx\Ind$ was unmodulated but subject to block fading. By coding across many such blocks, the information rate $\EVVar{v\Tx\Ind}{\RateMaxGP}$ can be achieved \cite[Sec.~5.4.5]{Tse2005}. Thereby $\RateMaxGP$ is the complicated expression from \Cref{eq:Capacity}.

\textbf{3.) The ambient source is PSK modulated:} PSK has a constant envelope, so $|v\Tx\Ind|$ and $|v\Rx\Ind|$ are constant for the duration of a fading block. The phase shifts in $v$ due to $v\Tx\Ind$ can be compensated with the knowledge from the decoded $v\Rx\Ind$. Then the system behaves as if $v\Tx\Ind$ was constant.
